Event-assisted 12-stop HDR Imaging of Dynamic Scene

High dynamic range (HDR) imaging is a crucial task in computational photography, which captures details across diverse lighting conditions. Traditional HDR fusion methods face limitations in dynamic scenes with extreme exposure differences, as aligning low dynamic range (LDR) frames becomes challenging due to motion and brightness variation. In this work, we propose a novel 12-stop HDR imaging approach for dynamic scenes, leveraging a dual-camera system with an event camera and an RGB camera. The event camera provides temporally dense, high dynamic range signals that improve alignment between LDR frames with large exposure differences, reducing ghosting artifacts caused by motion. Also, a real-world finetuning strategy is proposed to increase the generalization of alignment module on real-world events. Additionally, we introduce a diffusion-based fusion module that incorporates image priors from pre-trained diffusion models to address artifacts in high-contrast regions and minimize errors from the alignment process. To support this work, we developed the ESHDR dataset, the first dataset for 12-stop HDR imaging with synchronized event signals, and validated our approach on both simulated and real-world data. Extensive experiments demonstrate that our method achieves state-of-the-art performance, successfully extending HDR imaging to 12 stops in dynamic scenes.

==> sec/0_abstract.tex <==
\begin{abstract}
High dynamic range (HDR) imaging is crucial in computational photography for capturing details across diverse lighting conditions. Traditional methods increase dynamic range by merging multiple low dynamic range (LDR) images at different exposures, but struggle with very high dynamic scenes due to alignment failures when handling large exposure differences and motion blur. To address these limitations, we propose a novel approach utilizing event cameras—neuromorphic sensors with dynamic range and are free of motion blur—to assist in frame alignment and deblurring~\tianfan{Shall we still mention motion blur and deblurring in the abstract?}. As result, we are the first to achieve HDR imaging for dynamic scenes across a 12-stop exposure range. To utilize event signal, we proposed a two-stage framework consists of a reconstruction module leveraging intra- and inter-exposure events for deblurring and alignment, followed by a fusion module using pretrained diffusion models for final HDR generation. We validate our approach using a simulation pipeline to generate dynamic HDR sequences and an RGB-event dual-camera system for real-world data, demonstrating significant improvements over traditional methods.
\end{abstract}






==> sec/0_abstract_v1.tex <==
\begin{abstract}
High dynamic range (HDR) imaging is crucial in computational photography for capturing details across diverse lighting conditions. Traditional methods increase dynamic range by merging multiple low dynamic range (LDR) images at different exposures, but struggle with very high dynamic scenes due to alignment failures when handling large exposure differences and motion blur. To address these limitations, we propose a novel approach utilizing event cameras—neuromorphic sensors with dynamic range and are free of motion blur—to assist in frame alignment and deblurring. As result, we are the first to achieve HDR imaging for dynamic scenes across a 12-stop exposure range. To utilize event signal, we proposed a two-stage framework consists of a reconstruction module leveraging intra- and inter-exposure events for deblurring and alignment, followed by a fusion module using pretrained diffusion models for final HDR generation. We validate our approach using a simulation pipeline to generate dynamic HDR sequences and an RGB-event dual-camera system for real-world data, demonstrating significant improvements over traditional methods  with the introduction of events.

\end{abstract}






==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

High dynamic range imaging (HDR) is a fundamental task in computational photography, aiming to accurately capture the full range of visual details in both bright and dark regions of a scene. Real-world scenes often exhibit a luminance range spanning 80 to 100 dB~\cite{xiao2002high,pattanaik1998multiscale}, far exceeding the capabilities of common imaging sensors due to physical limitations. HDR imaging has diverse applications, such as film production, virtual reality, and medical imaging, making it crucial for enhancing visual perception in challenging lighting conditions.

The most common approach to capture HDR images is to merge information from a sequence of low dynamic range (LDR) images taken at multiple exposure levels. Capturing HDR scenes (\eg, transitioning from indoor to outdoor or night scenes) typically requires 7 to 12 exposure stops to recover the entire dynamic range~\cite{barakat2008minimal}. For example,~\cite{gardner2017learning,hold2019deep} captured 7 bracketed exposures and merged them into a full HDR image. Several studies~\cite{mertens2007exposure,ma2015multi,kou2017multi,ma2019deep} have proposed to multi-exposure image fusion, but they often assume static scenes, limiting their applicability in dynamic environments. To address this, researchers have explored HDR imaging for dynamic scenes. A key challenge in HDR imaging for dynamic scenes is frame alignment. Methods like deformable convolution~\cite{liu2021adnet,chen2021hdr}, pyramid cross-attention modules~\cite{liu2023joint}, and flow estimation~\cite{kalantari2019deep,xu2024hdrflow} have been proposed to align frames effectively before merging. However, these approaches primarily focus on merging two or three exposure levels within a 6-stop range (\eg, -3 EV to +3 EV). Extending these methods to handle larger exposure brackets, such as 12 stops, remains challenging due to motion blur in longer exposure images and large content differences between high and low EV levels, which makes frame alignment difficult. These challenges raise an interesting question: \emph{Can we achieve 12-stop HDR imaging for dynamic scenes effectively?}

To tackle this challenge, we incorporate event cameras to assist in frame alignment and deblurring of long-exposure images. Event cameras~\cite{serrano2013128,brandli2014240} are neuromorphic sensors that record only pixel-wise brightness changes, providing microsecond-level temporal resolution and a high dynamic range ($>120 dB$). The high dynamic range of event signals allows for consistent motion information across different exposure times in both bright and dark regions. This information can be leveraged to assist in deblurring RGB images and aligning frames across different exposure levels. Previous event-assisted HDR methods~\cite{messikommer2022multi,shaw2022hdr,yang2023learning,xiaopeng2024hdr} typically follow the RGB HDR setting using 2-3 exposure RGB images. In this work, we aim to advance this further by exploring event-guided 12-stop HDR imaging for dynamic scenes.

However, using event signals to assist 12-stop HDR imaging presents numerous challenges. Firstly, multiple tasks must be addressed, including deblurring, denoising, alignment, and fusion. Although event signals provide sufficient motion information, designing an effective network for 12-stop HDR imaging is crucial. Thus, we propose a two-stage framework consisting of a reconstruction module and a fusion module. The reconstruction module uses intra-exposure events to assist in deblurring and inter-exposure events to assist in frame alignment, resulting in aligned LDR images at different exposure times. The second stage merges these LDR images into the final HDR image. To handle the large exposure range fusion and reduce the impact of errors from the first stage on the final fusion, we utilize pretrained diffusion models as priors and designed a diffusion-based fusion module.

Furthermore, obtaining data for event-guided 12-stop HDR imaging is challenging. Traditional HDR training data simulation methods involve degrading LDR images to different exposures, which struggle to simulate complementary information from -6 EV to 6 EV. Additionally, the lack of high frame rate HDR video data makes event simulation difficult. To address these issues, we designed an event-assisted HDR simulation pipeline. Using HDR scene datasets and HDR object datasets, we simulate continuous motion to generate dynamic HDR sequences. We also simulate motion blur in the RAW domain by merging multiple frames and generate event signals in linear color space using V2E to simulate the entire imaging process. To validate our algorithm in real-world scenarios, we built an RGB-event dual-camera system capable of capturing sequences with triggers from -6 EV to 6 EV. Our experiments demonstrate the effectiveness of our approach on both simulated and real data.




==> sec/1_intro_v1.tex <==
\section{Introduction}
\label{sec:intro}

High dynamic range (HDR) imaging is an important task in computational photography, aiming to accurately capture the full range of visual details in both bright and dark regions of a scene. Real-world scenes often exhibit luminance levels spanning 80 to 100 dB~\cite{xiao2002high,pattanaik1998multiscale}, which far exceed the capabilities of conventional imaging sensors due to physical limitations. HDR imaging plays a critical role in applications such as film production, virtual reality, and medical imaging, enhancing visual perception under challenging lighting conditions.

The most common approach to HDR imaging is to merge information from multiple low dynamic range (LDR) images taken at different exposure levels. Capturing complex HDR scenes (\eg, transitioning between indoor and outdoor settings or night scenes) typically requires 7 to 12 exposure stops to recover the entire dynamic range~\cite{barakat2008minimal}. However, while several studies~\cite{gardner2017learning,hold2019deep} have used 7 bracketed exposures to construct full HDR images, handling such wide exposure brackets presents unique challenges. Conventional methods based on multi-exposure fusion~\cite{mertens2007exposure,ma2015multi,kou2017multi,ma2019deep} perform well under static scenes but struggle in dynamic environments. When applied to dynamic scenes, frame alignment becomes essential to prevent ghosting artifacts. Existing solutions—such as deformable convolutions~\cite{liu2021adnet,chen2021hdr}, pyramid cross-attention modules~\cite{liu2023joint}, and optical flow-based alignment~\cite{kalantari2019deep,xu2024hdrflow}—primarily handle 2-3 exposure images within a 6-stop range (e.g., -3 EV to +3 EV). Extending these techniques to a 12-stop range, from -6 EV to +6 EV, introduces new difficulties, as the large exposure gaps lead to misalignments and significant motion blur. These challenges raise a central question: \emph{Can we push HDR imaging to 12 stops in dynamic scenes effectively?}

Recent works have explored event-based cameras (EBCs) as an additional modality for HDR imaging~\cite{messikommer2022multi,shaw2022hdr,yang2023learning}. However, these studies typically focus on merging RGB exposures directly from event streams or use event-guided alignment on 2-3 exposure images, without addressing the larger challenges of extending the HDR range to 12 stops. Importantly, existing methods fall short in tackling the fundamental limitations of event-based imaging: noisy event streams and insufficient spatial resolution, which compromise the accuracy of HDR reconstructions. Instead of relying on events alone to generate HDR, our approach leverages events as an auxiliary signal to solve two critical problems that hinder traditional HDR: accurate alignment and deblurring of large exposure brackets.

In this work, we introduce a new paradigm for HDR imaging that integrates event streams with bracketed exposures to extend the HDR range to 12 stops. Our key insight is that events complement RGB exposures by providing fine-grained motion information across both bright and dark regions, enabling precise alignment and effective deblurring that cannot be achieved with RGB inputs alone. Specifically, we design a two-stage framework that addresses the major bottlenecks in dynamic HDR imaging. In the first stage, intra-exposure events are used to assist in deblurring, while inter-exposure events provide information for frame alignment across exposure levels. This alignment ensures that LDR images from -6 EV to +6 EV are consistently aligned, avoiding ghosting and improving temporal coherence. In the second stage, we introduce a diffusion-based fusion module that merges the aligned LDR images into a final HDR output. The diffusion model acts as a robust prior, mitigating errors from the alignment process and enhancing the fusion across such a wide dynamic range.

Obtaining training data for 12-stop HDR imaging with events poses another major challenge. Traditional HDR simulation methods degrade LDR images to approximate multiple exposures but fail to replicate the complementary information needed across -6 EV to +6 EV accurately. Furthermore, the lack of high frame rate HDR video data complicates the simulation of realistic event streams. To address these gaps, we developed a custom HDR simulation pipeline that combines HDR scene datasets and HDR object datasets to generate dynamic HDR sequences. This pipeline simulates motion blur directly in the RAW domain by merging frames and generates event signals in linear color space using V2E. This approach allows us to faithfully model the complete imaging process, capturing both RGB exposures and events in sync.

To validate our approach, we built an RGB-event dual-camera system capable of capturing synchronized sequences across a -6 EV to +6 EV range. This system ensures precise temporal alignment between events and RGB images, enabling real-world testing of our algorithm. Our extensive experiments on both simulated and real-world datasets demonstrate that our framework achieves state-of-the-art performance across challenging dynamic scenes, successfully pushing HDR imaging to a 12-stop range.




==> sec/1_intro_v2.tex <==

\section{Introduction}
\label{sec:intro}
High dynamic range (HDR) imaging is a fundamental task in computational photography, aiming to accurately capture the full range of visual details in both bright and dark regions of a scene. HDR imaging plays a critical role in applications such as film production, virtual reality, and medical imaging, enhancing visual perception under challenging lighting conditions. Real-world scenes often exhibit luminance levels spanning 80 to 100 dB~\cite{xiao2002high,pattanaik1998multiscale}, which far exceed the capabilities of conventional imaging sensors due to physical limitations. 

The most common approach to HDR imaging involves merging complementary information from multiple low dynamic range (LDR) images captured at varying exposure levels. Complex HDR scenes (\eg, transitions between indoor and outdoor settings or night scenes) typically require 7 to 12 exposure stops to fully recover the dynamic range~\cite{barakat2008minimal,gardner2017learning,hold2019deep}. Static multi-exposure fusion methods~\cite{mertens2007exposure,ma2015multi,kou2017multi,ma2019deep} can achieve a 12-stop HDR, but they do not account for motion in the scene or camera shake, making them unsuitable for dynamic scenes and thus limiting their applicability (see Fig.~\ref{fig:teaser} (c)). While dynamic HDR methods~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow} incorporate frame alignment modules to handle HDR in dynamic scenes. However, due to the lack of motion information between LDR frames, image alignment becomes challenging when dealing with complex motion and large exposure differences between LDR images, as this leads to substantial differences in image content. As a result, previous dynamic HDR methods are restricted to handling only 2–3 exposure images within a 6-stop range (e.g., -3 EV to +3 EV), leading to information loss in high-contrast scenes (see Fig.~\ref{fig:teaser} (d)). This raises an important and interesting question: \emph{Is it possible to extend HDR imaging to 12 stops in dynamic scenes?}

Frame alignment is a key challenge in dynamic-scene 12-stop HDR imaging due to large exposure variability. We propose a dual-camera system with an event camera~\cite{serrano2013128,brandli2014240} and a conventional RGB camera to address alignment problem. Event cameras capture pixel-level intensity changes, producing temporally dense event streams with a high dynamic range (approximately 140 dB). As shown in Fig.~\ref{fig:teaser} (b), event signals provide consistent, fine-grained motion information across both bright (+6 EV LDRs) and dark (-6 EV LDRs) regions. This helps mitigate discrepancies between LDR frames with different exposures and provides crucial motion information for accurate alignment. Our approach explicitly uses event signals to assist in 12-stop HDR alignment. Unlike previous works~\cite{messikommer2022multi,shaw2022hdr}, which implicitly use event data for 4-6 stop HDR alignment, struggling with large motion resulting in ghosting artifacts (see Fig.~\ref{fig:teaser} (e)), our method explicitly estimates optical flow to reduce these artifacts in scenes with large exposure differences. Moreover, to bridge the domain gap between synthetic and real event data, we fine-tune our model on extensive real-world Event-RGB interpolation datasets, enhancing the alignment module's robustness in real-world scenes.

Another challenge for dynamic-scene 12-stop HDR imaging is the fusion module for LDR images with extreme exposure differences. Due to the extremely high dynamic range of 12-stop HDR, many details are compressed into a very narrow value range, and there is a lack of a well-generalizable differentiable tone mapping method that can effectively handle both bright and dark regions. Current learning-based HDR imaging methods~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow} use the $\mu$-law tone mapping as a loss function, which often results in artifacts when using in 12-stop HDR. Additionally, the alignment process for 12-stop HDR inevitably introduces artifacts, occlusions, and errors, further complicating the fusion process. To address these issues, we design a diffusion-based fusion module that incorporates image priors from pre-trained diffusion models to reduce error accumulation from the alignment module and mitigate artifacts in areas where texture details are compressed.

Furthermore, to address the lack of datasets for 12-stop HDR imaging with event signals, we designed a simulation pipeline and developed the first dataset for dynamic-scene 12-stop HDR imaging with synchronized event signals, denoted as the ESHDR dataset, for training and evaluation. Compared with previous HDR simulation pipelines~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow}, which simulate multiple exposure LDRs from LDR images, our simulation pipeline generates LDR images from -6 to +6 EV using dynamic HDR scenes by combining HDR scene datasets and HDR object datasets to create dynamic HDR sequences, ensuring sufficient effective information at extreme EV levels. This pipeline simulates events using V2E while also considering LDR degradations, such as noise and blur. To validate our methods in real-world scenarios, we built an RGB-event dual-camera system capable of capturing synchronized sequences across a -6 EV to +6 EV range. Extensive experiments on both simulated and real-world datasets demonstrate that our framework achieves state-of-the-art performance across challenging dynamic scenes, successfully pushing HDR imaging to a 12-stop range.

Our key contributions are summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, we make the first attempt at 12-stop HDR imaging for dynamic scenes.

    \item We propose an event-assisted diffusion-based HDR method that focuses on solving two major challenges in dynamic-scene 12-stop HDR imaging: image alignment and fusion for LDRs with extreme exposure differences.

    \item We develop the first dataset, ESHDR, for 12-stop HDR imaging with event signals, and build a dual-camera system to validate our approach on both simulated and real-world datasets, demonstrating the practical feasibility and effectiveness of our method.
\end{itemize}

(Add a syn/real figure->alignment and fusion.)

==> sec/1_intro_v5.tex <==

\section{Introduction}
\label{sec:intro}
High dynamic range (HDR) imaging is a fundamental task in computational photography, aiming to accurately capture the full range of visual details in both bright and dark regions of a scene. HDR imaging plays a critical role in applications such as film production, virtual reality, and medical imaging, enhancing visual perception under challenging lighting conditions. Real-world scenes often exhibit luminance levels spanning 80 to 100 dB~\cite{xiao2002high,pattanaik1998multiscale}, which far exceed the capabilities of conventional imaging sensors due to physical limitations. 

The most common approach to HDR imaging involves merging complementary information from multiple low dynamic range (LDR) images captured at varying exposure levels. Complex HDR scenes (\eg, transitions between indoor and outdoor settings or night scenes) typically require 7 to 12 exposure stops to fully recover the dynamic range~\cite{barakat2008minimal,gardner2017learning,hold2019deep}. Static multi-exposure fusion methods~\cite{mertens2007exposure,ma2015multi,kou2017multi,ma2019deep} can achieve a 12-stop HDR, but they do not account for motion in the scene or camera shake, making them unsuitable for dynamic scenes and thus limiting their applicability (see Fig.~\ref{fig:teaser} (c)). While dynamic HDR methods~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow} incorporate frame alignment modules to handle HDR in dynamic scenes. However, due to the lack of motion information between LDR frames, image alignment becomes challenging when dealing with complex motion and large exposure differences between LDR images, as this leads to substantial differences in image content. As a result, previous dynamic HDR methods are restricted to handling only 2–3 exposure images within a 6-stop range (e.g., -3 EV to +3 EV), leading to information loss in high-contrast scenes (see Fig.~\ref{fig:teaser} (d)). This raises an important and interesting question: \emph{Is it possible to extend HDR imaging to 12 stops in dynamic scenes?}

Frame alignment is a key challenge in dynamic-scene 12-stop HDR imaging due to large exposure variability. We propose a dual-camera system with an event camera~\cite{serrano2013128,brandli2014240} and a conventional RGB camera to address alignment problem. Event cameras capture pixel-level intensity changes, producing temporally dense event streams with a high dynamic range (approximately 140 dB). As shown in Fig.~\ref{fig:teaser} (b), event signals provide consistent, fine-grained motion information across both bright (+6 EV LDRs) and dark (-6 EV LDRs) regions. This helps mitigate discrepancies between LDR frames with different exposures and provides crucial motion information for accurate alignment. Our approach explicitly uses event signals to assist in 12-stop HDR alignment. Unlike previous works~\cite{messikommer2022multi,shaw2022hdr}, which implicitly use event data for 4-6 stop HDR alignment, struggling with large motion resulting in ghosting artifacts (see Fig.~\ref{fig:teaser} (e)), our method explicitly estimates optical flow to reduce these artifacts in scenes with large exposure differences. Moreover, to bridge the domain gap between synthetic and real event data, we fine-tune our model on extensive real-world Event-RGB interpolation datasets, enhancing the alignment module's robustness in real-world scenes.

Another challenge for dynamic-scene 12-stop HDR imaging lies in the fusion module, which need effectively combine LDR images with extreme exposure differences. Firstly, the fusion module requires strong image priors to minimize artifacts. Due to the extremely high dynamic range of 12-stop HDR, many details are compressed into a very narrow value range, which causes even small discrepancies in the fusion output to result in significant artifacts after tone mapping. To address this issue, current learning-based HDR imaging methods~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow} employ $\mu$-law tone mapping as a loss function to enhance the value differences between details. However, the $\mu$-law function alone is insufficient for effectively managing both bright and dark regions in 12-stop HDR. Moreover, the fusion module must also mitigate the error accumulation inherent in the alignment process for 12-stop HDR, which inevitably introduces artifacts, occlusions, and errors. To tackle these challenges, we propose a diffusion-based fusion module that integrates image priors from pre-trained diffusion models to reduce error accumulation from the alignment module and mitigate artifacts in regions where texture details are highly compressed (see Fig.~\ref{fig:teaser} (f)).

Furthermore, to address the lack of datasets for 12-stop HDR imaging with event signals, we designed a simulation pipeline and developed the first dataset for dynamic-scene 12-stop HDR imaging with synchronized event signals, denoted as the ESHDR dataset, for training and evaluation. Compared with previous HDR simulation pipelines~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow}, which simulate multiple exposure LDRs from LDR images, our simulation pipeline generates LDR images from -6 to +6 EV using HDR scenes, ensuring sufficient effective information at extreme EV levels. To validate our methods in real-world scenarios, we built an RGB-event dual-camera system capable of capturing synchronized Event and RGB sequences across a -6 EV to +6 EV range. Extensive experiments on both simulated and real-world datasets demonstrate that our framework achieves state-of-the-art performance across challenging scenes, successfully pushing dynamic HDR imaging to a 12-stop range.

Our key contributions are summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, we make the first attempt at 12-stop HDR imaging for dynamic scenes.

    \item We propose an event-assisted diffusion-based HDR method that focuses on solving two major challenges in dynamic-scene 12-stop HDR imaging: image alignment and fusion for LDRs with extreme exposure differences.

    \item We develop the first dataset, ESHDR, for 12-stop HDR imaging with event signals, and build a dual-camera system to validate our approach on both simulated and real-world datasets, demonstrating the practical feasibility and effectiveness of our method.
\end{itemize}

(Add a syn/real figure->alignment and fusion.)

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related-work}

\begin{figure*}[!t]
    %\setlength{\abovecaptionskip}{-0.10cm}
    %\setlength{\belowcaptionskip}{-0.7cm}
    \centering
    %\vspace{0.1cm}
    \begin{overpic}[width=1\textwidth]{images/framework_v6.png}
    \end{overpic}

    \caption{Illustration of the framework of our network~\tianfan{Too many notations, like $E(t_1)$, in this diagram. Try to make it simple.}.}
    \label{fig:main-network}
\end{figure*}

\subsection{RGB-based HDR Imaging}
The objective of High Dynamic Range (HDR) imaging is to capture scenes with a broad dynamic spectrum, addressing the limitations of standard digital cameras, which typically exhibit a dynamic range around 70dB. The previous method for achieving HDR imaging involves merging multiple Low Dynamic Range (LDR) images taken at various exposure levels. This approach presents challenges, especially due to motion in dynamic scenes and variations in noise levels across exposures, often leading to ghosting artifacts~\cite{hu2013hdr,oh2014robust}. Traditional techniques~\cite{hu2013hdr,ma2017robust,oh2014robust,sen2012robust,mangiat2010high} have focused on mitigating these artifacts through complex image alignment methods. Kalantari \emph{et al.} \citet{kalantari2013patch} introduced a patch-based synthesis technique for HDR images to enhance temporal continuity by enforcing similarity across adjacent frames.

Recent advancements in deep learning have seen methods that employ Convolutional Neural Networks (CNNs) to map LDR images to tonemapped HDR outputs directly. Several approaches~\cite{wu2018deep,yan2019attention,yan2022dual,liu2022ghost,chen2022attention} circumvent the need for explicit alignment by incorporating an attention mechanism to address ghosting artifacts. \cite{yan2019attention,yan2022dual} have refined this strategy by introducing a context-aware transformer designed to improve model performance in complex dynamic scenes. Furthermore, some methods~\cite{liu2021adnet,chen2021hdr,liu2023joint,yan2023unified,chung2023lan,kalantari2019deep,xu2024hdrflow} continue to enhance alignment within deep learning frameworks. For instance, deformable convolutions~\cite{liu2021adnet,chen2021hdr} and more complex models like the pyramid cross-attention module~\cite{liu2023joint} and the content alignment model~\cite{yan2023unified}, which integrates ghost attention and patch aggregation, have been employed. Additionally, \cite{chung2023lan} explored frame alignment using a luminance-based attention score, while \cite{kalantari2019deep,xu2024hdrflow} proposed estimating motion flow from LDRs to facilitate alignment through warping operations.

Despite these improvement, existing RGB-based HDR methods typically utilize two or three exposures, a limitation that restricts their effectiveness in scenes with ultra-high dynamic ranges. Earlier methods~\cite{gardner2017learning,hold2019deep} captured seven exposures using a tripod to record the full unsaturated dynamic range but were limited to static scenes. The motion blur associated with long exposures and the challenges of aligning LDRs across a broad range of exposures complicate the capture of ultra-high dynamic range images in dynamic scenes.

Given the ultra-high dynamic range capabilities of event cameras, this paper investigates the challenging task of ultra-high dynamic range imaging in dynamic scenes, utilizing both RGB and event cameras.

\subsection{Event-based HDR Imaging}
Inspired by the human visual system, event sensors~\cite{serrano2013128,brandli2014240} measure the intensity changes per pixel and output temporally dense but spatially sparse event streams. These event signals boast a high dynamic range (approximately 140dB) with remarkable temporal precision, often operating at the microsecond level. Consequently, event-based HDR imaging has emerged as an increasingly attractive research field~\cite{wang2019event,rebecq2019high,yang2023learning,messikommer2022multi,shaw2022hdr,xiaopeng2024hdr}.

One type of approach involves directly utilizing the high dynamic range of the event signal to generate HDR RGB video through generative adversarial networks~\cite{wang2019event} and recurrent networks~\cite{rebecq2019high}. However, the absence of spatially dense RGB signals often results in suboptimal quality. Consequently, \citet{yang2023learning} leverage the event signal to guide the reconstruction of HDR images from LDR counterparts. \citet{xiaopeng2024hdr} further address motion blur and propose a self-supervised framework. Nonetheless, relying solely on RGB images with a single exposure fails to fully capture the entire exposure range. 

Other methods incorporate multi-exposure LDRs, similar to RGB-based HDR reconstruction, and employ event signals to facilitate the alignment process of LDRs~\cite{messikommer2022multi,shaw2022hdr}. \citet{messikommer2022multi} utilize deformable convolutions for alignment, while Shaw \emph{et al.}~\citet{shaw2022hdr} introduce an event-to-image feature distillation module to translate event features into the image domain.

Despite these advancements, merging only three exposures with four stops fails to fully exploit the ultra-high dynamic range (approximately 120dB) offered by event signals. Therefore, in this paper, we advance the study of ultra-high dynamic range imaging by employing seven exposures spanning 12 stops.

==> sec/2_related_v1.tex <==
\begin{figure*}[!t]
    %\setlength{\abovecaptionskip}{-0.10cm}
    %\setlength{\belowcaptionskip}{-0.7cm}
    \centering
    %\vspace{0.1cm}
    \begin{overpic}[width=1\textwidth]{images/framework_v7.png}
    \end{overpic}

    \caption{Illustration of the framework of our network~\tianfan{Too many notations, like $E(t_1)$, in this diagram. Try to make it simple.}.}
    \label{fig:main-network}
\end{figure*}

\section{Related Work}
\label{sec:related-work}



\subsection{RGB-based HDR Imaging}
The objective of High Dynamic Range (HDR) imaging is to capture scenes with a broad dynamic spectrum, addressing the limitations of standard digital cameras, which typically exhibit a dynamic range around 70dB. The previous method for achieving HDR imaging involves merging multiple Low Dynamic Range (LDR) images taken at various exposure levels. This approach presents challenges, especially due to motion in dynamic scenes and variations in noise levels across exposures, often leading to ghosting artifacts~\cite{hu2013hdr,oh2014robust}. Traditional techniques~\cite{hu2013hdr,ma2017robust,oh2014robust,sen2012robust,mangiat2010high} have focused on mitigating these artifacts through complex image alignment methods. Kalantari \emph{et al.} \citet{kalantari2013patch} introduced a patch-based synthesis technique for HDR images to enhance temporal continuity by enforcing similarity across adjacent frames.

Recent advancements in deep learning have seen methods that employ Convolutional Neural Networks (CNNs) to map LDR images to tonemapped HDR outputs directly. Several approaches~\cite{wu2018deep,yan2019attention,yan2022dual,liu2022ghost,chen2022attention} circumvent the need for explicit alignment by incorporating an attention mechanism to address ghosting artifacts. \cite{yan2019attention,yan2022dual} have refined this strategy by introducing a context-aware transformer designed to improve model performance in complex dynamic scenes. Furthermore, some methods~\cite{liu2021adnet,chen2021hdr,liu2023joint,yan2023unified,chung2023lan,kalantari2019deep,xu2024hdrflow} continue to enhance alignment within deep learning frameworks. For instance, deformable convolutions~\cite{liu2021adnet,chen2021hdr} and more complex models like the pyramid cross-attention module~\cite{liu2023joint} and the content alignment model~\cite{yan2023unified}, which integrates ghost attention and patch aggregation, have been employed. Additionally, \cite{chung2023lan} explored frame alignment using a luminance-based attention score, while \cite{kalantari2019deep,xu2024hdrflow} proposed estimating motion flow from LDRs to facilitate alignment through warping operations.

Despite these improvement, existing RGB-based HDR methods typically utilize two or three exposures, a limitation that restricts their effectiveness in scenes with ultra-high dynamic ranges. Earlier methods~\cite{gardner2017learning,hold2019deep} captured seven exposures using a tripod to record the full unsaturated dynamic range but were limited to static scenes. The motion blur associated with long exposures and the challenges of aligning LDRs across a broad range of exposures complicate the capture of ultra-high dynamic range images in dynamic scenes.

Given the ultra-high dynamic range capabilities of event cameras, this paper investigates the challenging task of ultra-high dynamic range imaging in dynamic scenes, utilizing both RGB and event cameras.

\subsection{Event-based HDR Imaging}

Event-based imaging, inspired by the human visual system, captures pixel-level intensity changes with exceptional temporal precision, offering a dynamic range up to 140 dB~\cite{serrano2013128, brandli2014240}. This high temporal resolution makes event cameras ideal for high-dynamic-range (HDR) imaging in dynamic and rapidly changing scenes, addressing the limitations of traditional HDR methods that struggle with motion blur, exposure misalignment, and slow temporal response~\cite{wang2019event, rebecq2019high, shaw2022hdr}. Early works explored generating HDR videos directly from event streams, using generative adversarial networks (GANs)~\cite{wang2019event} and recurrent networks~\cite{rebecq2019high}, though these approaches were limited by the sparse spatial resolution of event data. To overcome this, recent methods have combined event data with low dynamic range (LDR) images to enhance HDR reconstruction. For example, Yang \textit{et al.}~\cite{yang2023learning} incorporated event signals to guide the reconstruction of HDR images from LDR frames, improving image quality in dynamic environments, while Xiaopeng \textit{et al.}~\cite{xiaopeng2024hdr} introduced a self-supervised framework leveraging event data for motion compensation, significantly reducing motion blur in HDR reconstruction.

Recent approaches have extended event-based HDR methods by integrating multi-exposure LDR images alongside event data. Messikommer \textit{et al.}~\cite{messikommer2022multi} utilized deformable convolutions to align multi-exposure LDR frames, while Shaw \textit{et al.}~\cite{shaw2022hdr} proposed an event-to-image feature distillation module for better fusion of event data with RGB images. However, these methods typically use a limited number of exposures, restricting the full utilization of event cameras’ ultra-high dynamic range. In contrast, Li \textit{et al.}~\cite{li2024generalizing} presented a novel framework that combines single-exposure LDR images with event data, employing an Exposure Attention Fusion Module to adaptively merge multi-modal data and improve HDR quality across varying exposures. They also introduced a self-supervised EDDN loss, which enhances details in saturated regions while mitigating noise in underexposed areas, setting a new standard for event-based HDR imaging.

Recent works have also explored event-based HDR video reconstruction. Zou \textit{et al.}~\cite{zou2024eventhdr} proposed a recurrent convolutional network to reconstruct high-speed HDR videos from event data, incorporating a key-frame guidance mechanism to address the sparsity of event data. Wu \textit{et al.}~\cite{wu2024event} introduced the AsynHDR system, combining event cameras with LCD panels to modulate incident light, allowing passive HDR imaging in real-world environments. Additionally, Li \textit{et al.}~\cite{li2024ers} presented the ERS-HDRI framework for remote sensing applications, integrating event data with LDR images for HDR reconstruction, achieving a 30\% improvement in PSNR and 9\% in SSIM over existing methods. Finally, Chang \textit{et al.}~\cite{chang20231000} introduced a Spike-RGB hybrid camera system that captures high-speed HDR video at 1000 FPS, overcoming the limitations of conventional frame-based HDR cameras in fast-moving scenes.

In summary, while event-based HDR imaging has made significant advances, challenges remain in fully exploiting the high dynamic range and temporal precision of event cameras. Our work addresses these challenges by leveraging a multi-exposure strategy and diffusion priors for HDR fusion, enabling the reconstruction of HDR images spanning a 12-stop dynamic range and pushing the boundaries of HDR imaging in dynamic environments and real-time applications.


==> sec/3_method.tex <==
\section{Method}


\subsection{Overall Framework}
This study tackles the complex problem of 12-stop high dynamic range (HDR) reconstruction from a sequence of \( n \) low dynamic range (LDR) images, \( \{I_1, I_2, \ldots, I_n\} \), each captured at distinct timestamps \( \{t_1, t_2, \ldots, t_n\} \) with corresponding exposure times \( \{\tau_1, \tau_2, \ldots, \tau_n\} \). Additionally, this sequence is supplemented by a continuous stream of events, \( \{E_i\}_{t_1}^{t_n} \), providing high dynamic range temporal detail. Our objective is to achieve exposure fusion and synthesize a 12-stop HDR image, selectively integrating fine details across exposures. The obtained HDR image aligns with the reference frame $I_{\text{ref}}$, identified at timestamp $t_{\text{ref}}$.

In contrast to previous methods in exposure fusion~\cite{mertens2007exposure,ma2015multi,kou2017multi,ma2019deep} and dynamic HDR imaging~\cite{kalantari2019deep,liu2021adnet,chen2021hdr,liu2023joint,xu2024hdrflow}, we introduce a novel approach capable of performing 12-stop HDR imaging in dynamic scenes. To address the inherent challenges—specifically, the frame alignment and fusion of LDR frames with substantial exposure variation—we propose leveraging HDR event signals to facilitate explicit frame alignment and reconstruction in Sec.~\ref{sec:event-assisted-reconstruction}. Additionally, we incorporate a diffusion-based fusion model to generate the 12-stop HDR image in Sec.~\ref{sec:diff_fusion}. By utilizing the image prior learned from a pre-trained diffusion model, our fusion process achieves enhanced visualization in regions where textures are compressed within a narrow dynamic range, while also mitigating alignment-related error accumulation. The overall pipeline is summarized in Fig.~\ref{fig:main-network}.

\subsection{Event-Assisted Reconstruction}
\label{sec:event-assisted-reconstruction}
An event camera captures changes in scene illumination as an asynchronous stream of events. Each event at a position $ \mathbf{u} = (x, y) $ is triggered when the relative change in intensity exceeds a contrast threshold $ c $:
\begin{equation}
    E_t = \begin{cases}
        1, & \text{if } \log(I_{t}) - \log(I_{t-\Delta t}) \geq c, \\ 
        -1, & \text{if } \log(I_{t}) - \log(I_{t-\Delta t}) \leq -c,\\        
        0, & \text{otherwise},
        \end{cases}       
\label{eq:normal_define_evs}
\end{equation}
where $E_t$ represents the polarity of the event, $I_{t}$ denotes the image intensity at time $t$, and $\Delta t$ is the interval since the last event at position $\mathbf{u}$. 

By recording illumination changes in the $\log$ domain, the event signal provides not only microsecond-level temporal resolution but also a high dynamic range reaching up to 140 dB. This enables the event signal to capture motion information between LDR images and to preserve details in both bright and dark regions of RGB images, spanning a range of -6 EV to 6 EV. We leverage this event signal to support frame alignment and, to mitigate the impact of LDR degradation, we also utilize events recorded within each exposure interval to assist in deblurring.

\textbf{Intra-exposure Reconstruction:}
For LDR (Low Dynamic Range) images captured with a short exposure time, noise is often introduced into the image. Conversely, LDR images captured with a longer exposure time tend to suffer from motion blur~\tianfan{May need one sample image to show motion blur. Ideally, also show how intra-component may resolve it.}. Both noise and blur can significantly degrade the quality of the final exposure fusion image. Therefore, the objective of intra-exposure reconstruction is to leverage each LDR image $I_n$ captured with an exposure time $\tau_n$ and the event signal generated during $\tau_n$, denoted as $E_{t_n \rightarrow t_n + \tau_n}$, to obtain a clean and sharp LDR image. A simple UNet architecture is employed to achieve this reconstruction, and the reconstructed frame $I^{r}_n$ is computed as follows:
%
\begin{equation}
I^{r}_n = \text{UNet}(I_n, E_{t_n \rightarrow t_n + \tau_n}).
\end{equation}
%
Since we employ a synthesized training data pipeline, the ground truth LDR image $\hat{I}_n$ is available for training. The loss function is defined as:
%
\begin{equation}
\mathcal{L}_{\text{intra}} = \sqrt{\Vert \hat{I}_n - I^{r}_n \Vert^2 + \epsilon^2},
\end{equation}
%
where $\sqrt{\Vert \hat{x} - x \Vert^2 + \epsilon^2}$ represents the Charbonnier penalty function, and $\epsilon$ is set to 0.001.


%\subsubsection{Inter-exposure Alignment}
\textbf{Inter-exposure Alignment:}
Given that motion exists between the reconstructed LDR images $I^{r}_n$, the inter-exposure alignment model aims to align each $I^{r}_n$ with the reference LDR $I^{r}_{\text{ref}}$. In this work, we select the 0 EV LDR as the reference frame. Since LDR images are captured with varying exposure times, the content between $I^{r}_n$ and $I^{r}_{\text{ref}}$ can differ significantly. Therefore, inter-exposure event signals, denoted as $E_{t_n \rightarrow t_{\text{ref}}}$, are utilized for alignment. ~\tianfan{Similarly, show how an example of how inter-exposure alignment helps.}

However, training an inter-exposure alignment model remains challenging, even with the inclusion of event signals. The primary difficulties arise from the limited availability of training data, which makes it challenging to train a robust event flow estimation network from scratch. Additionally, inaccuracies in flow estimation can introduce artifacts in the subsequent diffusion-based fusion module. \tianfan{Make a new paragraph here.} To address these issues, we first use an RGB-pretrained flow estimation model to obtain an initial coarse flow, and then perform flow estimation in the feature space. \tianfan{Maybe visualize that event can greatly improve accuracy of flow in one example.} 

The encoder features of the two LDR images are extracted as follows:
\begin{equation}
f_n = E(I^r_n), \quad f_{\text{ref}} = E(A(I^r_{\text{ref}}, n)),
\end{equation}
where $E(\cdot)$ represents the encoder, which consists of two residual blocks, and $A(\cdot)$ aligns the exposure of the LDRs. The exposure alignment is defined as $A(I^r_{\text{ref}}, n) = \Gamma(\Gamma(I^r_{\text{ref}}, 2.4) \cdot \tau_n / \tau_{\text{ref}}, 1/2.4)$, where $\Gamma(I^r_{\text{ref}}, 2.4)$ is the inverse gamma correction to convert the image into linear space. The flow in the feature space is then estimated as:
\begin{equation}
\text{flow}_c = \text{FNet}(f_n, f_{\text{ref}}, \text{flow}_i, E_{t_n \rightarrow t_{\text{ref}}}),
\end{equation}
where $\text{flow}_i$ is the initial flow estimated using the pre-trained RGB flow estimation model, RAFT~\tianfan{}. The final aligned frame is obtained by:
\begin{equation}
f^a_n = D(W(f_n, \text{flow}_c)),
\end{equation}
where $W(x, \text{flow}_c)$ performs backward warping using the optical flow, and $D(\cdot)$ denotes the decoder that converts the image features back into the image space. To further enhance the accuracy of flow estimation, $f_n$ and $f_{\text{ref}}$ are divided into four groups, and the flow is estimated separately for each group.

\subsection{Diffusion-based Fusion} 
\label{sec:diff_fusion}

\tianfan{This \cref{sec:diff_fusion} sounds like simply applying SD, which sounds not novel and boring. Better to elaborate why diffusion is critical in this case, and how to apply it, in an non-trivial way (like those details about tonemapping). Some example images might be helpful.}

With the LDR images $I^a_{n}$, each aligned to the reference frame, the next step involves converting these images into a tone-mapped HDR image using the exposure fusion module. A common approach for exposure fusion is to estimate a weight map to average these LDR images. However, given the wide range of exposure levels in our LDR images, a direct weighted sum of these images could result in undesirable artifacts. To produce visually pleasing tone-mapped images that accommodate a wide exposure range, we opt for a diffusion-based model to perform the exposure fusion.

We leverage a pre-trained stable diffusion model to serve as the image prior, using the LDR images as the condition to guide the fusion process. This ensures that the resulting image exhibits visually pleasing characteristics across the varied exposure levels. Following the ControlNet strategy, we update only the encoder portion of the model during training. The final fused image $I'$ is then obtained by~\tianfan{I did not find this equation useful. Consider to remove it.}:
\begin{equation}
I' = \text{SD}(I^a_{n}),
\end{equation}
where $\text{SD}$ denotes the stable diffusion model applied to the aligned LDR images.

%\begin{table*}[th]
%\centering
%\begin{tabular}{l|l|l|l|l}
%        & RGB Noise                 & RGB Blur                  & Single EV Range                            & Event                     \\ \hline
%HDRFlow & $\checkmark$ &                           & {[}0ev, -3ev{]}, {[}-2ev, 0ev, 2ev{]}      &                           \\
%HDRev   &                           &                           & Single EV                                  & $\checkmark$ \\ \hline
%Ours    & $\checkmark$ & $\checkmark$ & {[}-6ev, -4ev, -2ev, 0ev, 2ev, 4ev, 6ev{]} & $\checkmark$
%\\ \hline
%\end{tabular}
%\end{table*}

==> sec/4_datasim.tex <==
\section{RGB-EVS HDR Simulation Pipeline}

(Using table or text to )

Acquiring real-world HDR images and event-based (EVS) signals simultaneously from the same scene is a challenging task. Previous methods for HDR imaging and EVS often rely on simulated data to overcome these difficulties. To facilitate the generation of training and testing datasets, we have developed a more comprehensive simulation pipeline, as illustrated in Fig. \ref{fig:data_simulation}. The pipeline begins by simulating a dynamic scene in HDR, as detailed in Sec.\ref{sec:dy_hdr_sim}. This simulated dynamic HDR scene is then used to generate a sequence of degraded low dynamic range (LDR) images with varying exposures (see Sec.\ref{sec:d_ldr_sim}), as well as the corresponding event-based signals captured during this sequence (see Sec.\ref{sec:evs_sim}).


\begin{figure}[t!]
    \centering
\includegraphics[width=0.47\textwidth]{CVPR25_EVSUDR/images/data_sim_v3.png}
    \caption{Framework of high dynamic range images and event signal simulation. \tianfan{This figure is too small.}}
    \label{fig:data_simulation}
\end{figure}

\subsection{Dynamic HDR Sequence Simulation}
\label{sec:dy_hdr_sim}
To synthesize dynamic HDR scenes, previous methods, such as HDRFlow, typically convert an LDR video into an "HDR" video, which is then transformed back into LDR videos at different exposure values (EVs). However, this simulation approach has significant limitations. The actual dynamic range does not increase; the initial LDR video already contains all the available information, and the additional LDR videos do not contribute any new data. Furthermore, since our goal in this paper is to explore HDR imaging with a higher exposure dynamic range, the traditional method of simulating HDR from LDR struggles to effectively generate meaningful information at higher EV levels (e.g., +4EV/+6EV). \tianfan{Diagram to show the simulation process, or just use an example to show that (like original HDR images, simulated HDR motion, final RGB bursts and events, etc.}

To address these issues, we simulate directly from HDR data. This approach, however, introduces a new challenge: obtaining HDR videos is inherently difficult. To overcome this, we simulate a dynamic HDR sequence by introducing motion into single-frame HDR images. We utilize the HDR indoor \cite{gardner2017learning} and outdoor \cite{hold2019deep} datasets for training and testing purposes, respectively. Additionally, to simulate the motion of foreground objects, we employ the Objaverse dataset \cite{deitke2023objaverse}, which includes HDR object data, to model the foreground movement. 

For the subsequent simulation of LDR sequences and event-based signals, we use a high frame rate with minimal motion between frames. Given the continuity of motion, we simulate it using the following equation:
%
\begin{equation}
    s_{t+1} = \alpha s_t + (1 - \alpha) \cdot random(S),
\end{equation}
%
where $s_t$ represents the motion shift at time $t$, $random(S)$ is a randomly generated motion, and $\alpha$ is the motion smoothing coefficient.


\subsection{Degraded LDR Simulation}
\label{sec:d_ldr_sim}

\tianfan{Needs a transition between this and previous paragraph.}

Traditional HDR methods typically consider the noise present in LDR images but often neglect the simulation of blur, especially at high exposure values (EVs). However, motion blur is a common phenomenon, and accurately modeling blur in LDR images is crucial for realistic simulation. To generate more realistic degraded LDR images, we first unprocess the HDR images back to the RAW domain using the inverse image processing pipeline (ISP)~\cite{brooks2019unprocessing}. During the exposure time, the RAW images are averaged to simulate motion blur, with the addition of signal-dependent Poisson-Gaussian noise. 

Subsequently, based on the specified EV values, we perform quantization and clipping operations to simulate the HDR-to-LDR conversion, producing LDR RAW images at different EVs. Finally, these RAW images are processed through the ISP to convert them into LDR images corresponding to the different exposure values.


\subsection{Event Signal Simulation}
\label{sec:evs_sim}

For the simulation of event signals, we directly utilize the HDR sequence and employ the V2E framework, which aligns with the high dynamic range characteristics of event signals. By considering both the intra-exposure and inter-exposure intervals, we simulate the formation of motion blur in the LDR images during exposure and generate the corresponding event signals between different exposures.



==> sec/5_experiments.tex <==
\section{Experiments}

\begin{table*}[!t]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Comparison of different methods on HDR image quality metrics. Higher values indicate better performance for metrics marked with ($\uparrow$), while lower values are preferable for metrics marked with ($\downarrow$). Note that $\mu$-PSNR, $\mu$-SSIM, LPIPS, DISTS, and MANIQA are evaluated in the $\mu$-law tone-mapped domain.}
\label{tab:hdr_comparison}
\begin{tabular}{l|cccccc|c}
\hline
\textbf{Method} & \textbf{PSNR} & \textbf{SSIM} & \textbf{$\mu$-PSNR} ($\uparrow$) & \textbf{$\mu$-SSIM} ($\uparrow$) & \textbf{LPIPS} ($\downarrow$) & \textbf{DISTS} ($\downarrow$) & \textbf{MANIQA} ($\uparrow$) \\\hline
HDRFlow (3-stop)       & 31.34 & 0.9653 & 27.57 & 0.9131 & 0.1938 & 0.1729 & 0.2519 \\
HDRFlow (6-stop)      & 32.14 & 0.9689 & 28.70 & 0.9152 & 0.1655 & 0.1599 & 0.2581 \\
HDR-Transformer (6-stop) & 32.38 & 0.9700 & 29.06 & 0.9153 & 0.1710 & 0.1607 & 0.2470 \\
HDR-Fusion (12-stop) & 27.38 &0.9493 &23.14 &0.8275 &0.3383 &0.2388 &0.2369\\
\hline
HDRV* (single LDR, EVS)      & 30.81 & 0.9746 & 31.87 & 0.9533 & 0.1269 & 0.1443 & 0.2996 \\
Event-HDR* (6-stop, EVS) & 33.85 & 0.9857 & 34.43 & 0.9523 & 0.1190 & 0.1425 & 0.3050 \\
\hline
Ours* (12-stop, EVS)    & \textbf{38.25} & \textbf{0.9876} & \textbf{35.66} & \textbf{0.9541} & \textbf{0.1091} & \textbf{0.1187} & \textbf{0.3168} \\\hline
\end{tabular}
\end{table*}

\subsection{Experiment Details}
In our experiment, we train our network on the training set of ESHDR. The model is implemented using PyTorch. During training, we use the Adam optimizer~\cite{Kingma2014AdamAM} with learning rate of $1 \times 10^{-4}$. We first train the event-assisted alignment module to obtain aligned LDR images for different exposures. Then, we train the diffusion-based fusion module. To maintain the color fidelity of the output HDR images in ESHDR evaluation, we further fine-tune one layer of the VAE decoder for several steps, which we refer to as Ours*. More details are provided in the supplementary material.

\subsection{Baseline Methods}
To evaluate our model, we first compare it with state-of-the-art RGB dynamic scene HDR imaging methods, namely HDRFlow~\cite{xu2024hdrflow} and HDR-Transformer~\cite{liu2022ghost}. Since HDRFlow and HDR-Transformer can only fuse LDR images ranging from -3EV to 3EV, we also compare our approach with a state-of-the-art HDR fusion method, HDR-Fusion~\cite{debevec2023recovering}, which can process 12-stop HDR imaging. To avoid color shifts between different RGB HDR imaging methods, we align the colors of all results to the ground truth HDR using a 3D bilateral grid~\cite{wang2024bilateral}. For event-assisted HDR imaging methods, due to different experimental settings and the unavailability of released code, we re-trained HDRV~\cite{yang2023learning} and Event-HDR~\cite{messikommer2022multi} on our training set, which we denote as HDRV* and Event-HDR*. 
%It is worth noting that the original versions of HDRV and Event-HDR do not account for the blurring and noise effects present in LDR images.

\begin{figure*}[t!]
    \centering
\includegraphics[width=\textwidth]{CVPR25_EVSUDR/images/syn_1.jpg}
    \caption{Visual comparisons of different HDR imaging methods. Since visualizing both the darkest and brightest areas in a 12-stop HDR image is a challenging task, we utilize two tone mapping styles, namely \emph{Deep} and \emph{Interior}, using commercial HDR software (Photomatix) to better highlight details in the bright and dark regions for comparison.}
    \label{fig:exp_syn_1}
\end{figure*}

\subsection{ESHDR Dataset}
In Table~\ref{tab:hdr_comparison} and Fig.~\ref{fig:exp_syn_1}, we present the quantitative and visual comparison results on the test set of the ESHDR dataset. It can be observed that our method achieves the best performance in both fidelity metrics (PSNR and SSIM) and perceptual quality metrics (LPIPS~\cite{zhang2018perceptual}, DISTS~\cite{ding2020iqa}, and non-reference MANIQA~\cite{yang2022maniqa}). 

In Fig.~\ref{fig:exp_syn_1}, we also observe that using more LDR images for fusion allows HDRFlow (with -3EV to 3EV exposures) to achieve better results in bright regions compared to HDRFlow using 0EV to 3EV exposures. Although HDR-Fusion employs 12-stop LDR images for fusion, this method is limited to static scenes, resulting in ghosting artifacts in dynamic scenes. 
%Since these RGB HDR imaging methods do not effectively handle noise and blur, noticeable artifacts are present in their results.
For HDRV*, even though it utilizes high dynamic range event signals, relying on a single LDR image is insufficient to achieve visually pleasing results. For Event-HDR*, despite leveraging event signals and alternately exposed LDR images, it performs better than previous methods in HDR recovery. However, in scenes with extremely high dynamic ranges, many texture details are compressed into narrow regions when using the $\mu$-law function to compute the loss. As a result, although artifacts are not apparent under the unbrightened tone mapping style (\emph{Deep}), they become evident after brightening (\emph{Interior}).

With the natural image priors embedded in our diffusion-based approach, our HDR reconstruction effectively reduces artifacts in both bright and dark regions. Furthermore, thanks to the fusion of LDR images ranging from -6EV to 6EV, our method delivers superior results in extremely high dynamic range regions (\eg, the sun), achieving minimal overexposure in bright areas.
  






\subsection{Real-world Experiments}

\begin{figure*}[t!]
    \centering
\includegraphics[width=\textwidth]{CVPR25_EVSUDR/images/real_2.jpg}
    \caption{Visual comparisons of different HDR imaging methods on real-captured data. We utilize tone mapping in commercial HDR software (Photomatix) to better visualization. (Matrix)}
    \label{fig:exp_real_1}
\end{figure*}

(LED/)
